Color Matching Using Hypernetwork-Based Kolmogorov-Arnold Networks

We present cmKAN, a versatile framework for color matching. Given an input image with colors from a source color distribution, our method effectively and accurately maps these colors to match a target color distribution in both supervised and unsupervised settings. Our framework leverages the spline capabilities of Kolmogorov-Arnold Networks (KANs) to model the color matching between source and target distributions. Specifically, we developed a hypernetwork that generates spatially varying weight maps to control the nonlinear splines of a KAN, enabling accurate color matching. As part of this work, we introduce a first large-scale dataset of paired images captured by two distinct cameras and evaluate the efficacy of our and existing methods in matching colors. We evaluated our approach across various color-matching tasks, including: (1) raw-to-raw mapping, where the source color distribution is in one camera's raw color space and the target in another camera's raw space; (2) raw-to-sRGB mapping, where the source color distribution is in a camera's raw space and the target is in the display sRGB space, emulating the color rendering of a camera ISP; and (3) sRGB-to-sRGB mapping, where the goal is to transfer colors from a source sRGB space (e.g., produced by a source camera ISP) to a target sRGB space (e.g., from a different camera ISP). The results show that our method outperforms existing approaches by 37.3% on average for supervised and unsupervised cases while remaining lightweight compared to other methods. The codes, dataset, and pre-trained models are available at: https://github.com/gosha20777/cmKAN

==> sec/1_intro.tex <==
\section{Introduction and Related Work}
\label{sec:intro}

Camera Image Signal Processors (ISPs) consist of various modules that process input image colors to produce the final output \cite{nakamura2017image, heide2014flexisp, karaimer2016software, delbracio2021mobile, brown2023color}. These ISPs perform different color transformations that map the initial image colors from the camera's raw space -- defined by the camera's characteristics -- to standardized color spaces (\eg, CIE XYZ or linear sRGB), ultimately converting them to display standard color spaces (\eg, DCI P3, nonlinear sRGB, or sRGB for short) \cite{nakamura2017image, brown2023color}. As a result, the same scene can be captured by two different cameras, leading to variations in color output. This discrepancy arises from several factors, including the initial raw colors produced by the camera sensor and the diverse algorithms employed by ISPs, which can vary in accuracy and reflect the desired styles that the camera manufacturer aims for in the final image \cite{zhou2007image, nguyen2014raw, delbracio2021mobile, tseng2022neural}.  

Color matching, or more specifically color stabilization, aims to adjust the colors of an input image (source) to closely resemble the colors of a reference image (target) that captures the same scene \cite{AN1, AN2}. Typically, these images are taken by different cameras or by the same camera but in different color spaces \cite{AN2, finlayson2015color}. Color matching can thus be considered a subset of color transfer, focused specifically on aligning colors between source and target images. In contrast, color transfer generally involves images from different scenes \cite{faridul2014survey, lv2024color} and seeks to transfer the ``feel'' and ``look'' of the target image to the source image \cite{nguyen2014illuminant}, often resulting in extensive image recoloring \cite{afifi2019image}. Unlike color transfer, color matching emphasizes accurate color reproduction between target and source images depicting the same scene \cite{AN2}.


Color matching is beneficial in various applications within camera pipeline manufacturing and photo editing, including mapping colors between different color spaces (\eg, raw-to-sRGB \cite{ignatov2020replacing} or sRGB-to-raw \cite{punnappurath2021spatially, nam2022learning}), post-capture white-balance editing (\eg, \cite{afifi2019color, afifi2020deep}), reusing camera ISP color modules for previously unsupported cameras through raw-to-raw mapping (\eg, \cite{afifi2021semi, perevozchikov2024rawformer}), ensuring consistent color reproduction across dual-camera systems to improve image quality (\eg, \cite{wu2023efficient, lai2022face, alzayer2023dc2}), and enable seamless dual-camera zoom \cite{wu2025dual}. While access to both source and target images is feasible in certain scenarios (\eg, on-board camera sRGB-to-raw mapping \cite{punnappurath2021spatially} or dual-camera aligned image color mapping \cite{lai2022face, wu2025dual}), there are other situations where this condition is difficult to achieve (\eg, raw-to-raw mapping \cite{afifi2021semi}, raw-to-sRGB mapping \cite{ignatov2020replacing, schwartz2018deepisp}, color mapping to specific embedded photographic styles \cite{AN7, AN8}, or generic color enhancement \cite{liu20234d, conde2024nilut}). 

Most existing color matching and transfer techniques, however, assume access to both source and target images or colors (\eg, \cite{AN2, AN1, finlayson2017color, fairchild2008matching, reinhard2001color, pitie2005n, xiao2006color, pitie2007automated, rabin2014adaptive, chang2015palette, afifi2021histogan, ding2024regional, ke2023neural}), which limits the applicability of these algorithms. In this work, we propose cmKAN, a framework suitable for both online paired-based optimization (where both source and target images are available at inference time) and offline training (where the target image is not accessible at inference time). Additionally, our cmKAN can be trained in an unsupervised manner, making it practical for scenarios where obtaining paired training data is challenging. 

Our cmKAN model is based on Kolmogorov-Arnold Networks (KANs) \cite{AN6}, which inherently provide non-linear, spline-based processing of input features, making them particularly well-suited for non-linear color matching. While Multi-Layer Perceptrons (MLPs) and Convolutional (conv) networks can model non-linear mappings through fixed activation functions, such as ReLU or sigmoid, KANs have shown promising results in lightweight, non-linear mappings between source and target distributions \cite{AN6}. KANs leverage spline-based activation functions, which are piecewise polynomials that allow more nuanced and flexible approximations of complex functions. In color processing, splines are commonly employed -- typically through closed-form fitting -- for color calibration \cite{menesatti2012rgb, tocci2022advantages, suominen2024camera}. This motivated us to integrate KANs into our color-matching framework, where we introduce a hypernetwork-based architecture that includes a generator to control the coefficients of the KAN splines. Acting as a hypernetwork \cite{ha2016hypernetworks}, the generator produces spatial weights that dictate the behavior of the KAN, enabling dynamic adaptation for color-matching tasks (see Fig.~\ref{fig:teaser}). 


We evaluated our framework on different tasks relevant to camera ISP development and post-capture editing. Specifically, we tested our approach on unsupervised raw-to-raw mapping, where the goal is to transform the raw colors from a source camera to resemble those produced by another camera in its raw space \cite{afifi2021semi}. Additionally, we examined raw-to-sRGB mapping, aiming to map images from the camera raw space to the standard display sRGB space (acting as a learnable camera ISP \cite{zhang2021learning, xing2021invertible, ignatov2020aim} from color perspective) using supervised training. Furthermore, we tested our framework on color mapping in the sRGB space, where the goal is to map the sRGB colors from the source camera to appear consistent with those from the target camera. For this task, we evaluated both unsupervised training (when no paired dataset is available) and supervised training. Additionally, we considered the scenario where both source and target images are available at inference. This situation applies to dual-camera-based processing (\eg, \cite{wu2023efficient, lai2022face, wu2025dual}) or for creating small learned metadata (\ie, in our case, the model's weights) to store for post-capture editing (\eg, \cite{afifi2019color, le2023gamutmlp}).

To evaluate our method's effectiveness in sRGB-to-sRGB color mapping between two different camera ISPs, we introduce a large dataset of 2.5K well-aligned paired images captured by two distinct cameras. We believe this dataset will be a valuable resource for evaluating color-matching techniques in future research. The code, trained models, and dataset will be made publicly available upon acceptance.

\subsection*{Contribution}
Our contributions can be summarized as follows:
\begin{itemize}
 

   \item  We propose \emph{cmKAN}, a lightweight hypernetwork-based framework for color matching using KANs. To the best of our knowledge, this is the first work to leverage the spline non-linearity in KANs for highly accurate, non-linear color matching.



   \item We present a large-scale dataset of paired, well-aligned images taken by two different cameras, facilitating the training and evaluation of color-matching methods.


   \item Our experimental results show that our method achieves state-of-the-art performance in color matching across multiple tasks (\ie, \emph{raw-to-raw}, \emph{raw-to-sRGB}, and \emph{sRGB-to-sRGB}) under unsupervised, supervised, and pair-based optimization schemes, while remaining lightweight and suitable for on-device applications.%". Furthermore, it remains lightweight and practical for on-device applications with limited computational power.
\end{itemize}

==> sec/3_proposed.tex <==
\section{Method}
\label{sec:method}
In this section, we outline the core principles of our proposed color-matching model using KANs -- cmKAN. As demonstrated in Fig.~\ref{fig:overview} (a), the cmKAN primarily comprises of a generator and a KAN network.  %presents an overview of our proposed cmKAN for color matching.
%As shown, our method includes a 
The generator network, acting as a hypernetwork, takes a source input image and produces a set of spatially varying %coefficient%
parameter maps in the latent space. These parameter maps are then used %to control the spline curves of our KAN network, 
as coefficients for basis splines of the KAN,
which adjusts the input image colors to match the target colors.

Without loss of generality, we assume that the input and target colors come from the source and target cameras, respectively, each of which may have its own ISP, leading to disparities in the final sRGB images we aim to match. For other scenarios (i.e., raw-to-sRGB or raw-to-raw mapping), the same model applies, where we learn to model the non-linear mapping between two different color spaces either within the same camera (raw-to-sRGB) or cross-cameras (raw-to-raw). We will first discuss in detail the core components of our color matching framework in Secs.~\ref{sec:generator} and \ref{sec:kan}. Then, we adopt the offline training scenario in Sec.~\ref{sec:supervised} and Sec.~\ref{sec:unsupervised}, and in Sec.~\ref{sec:optimization}, we explain how the proposed model can be used in a paired-based optimization scenario. %We will first discuss in detail the basic idea of cmKAN, then  the core components of our color matching framework in Secs.~\ref{sec:generator} and \ref{sec:kan}. Then, we adopt the offline training scenario in Sec.~\ref{sec:supervised} and Sec.~\ref{sec:unsupervised}, and in Sec.~\ref{sec:optimization}, we explain how the proposed model can be used in a paired-based optimization scenario.

%\subsection{Spatially parametrized KAN for Color Matching}
%\label{sec:cmKAN_idea}
%According to a several works ~\cite{AN1}, ~\cite{AN9} rendering of the source and target image by different camera ISPs from linear sensor response colors $ {I}_{lin} $ in standard device-independent color space, e.g. XYZ ~\cite{AN3} can be formulated as:
%\begin{equation}\label{eq1}
%{I}_{rdr}=T(w(\mathbf{x}))({I}_{in}\mathbf{C(\mathbf{x})}).
%\end{equation}
%Where matrix $\mathbf{C}$ represents linear part of the ISP pipeline, including white balancing and of color correction matrix, nonlinear transform ${T}$ implements nonlinear part like tone mapping and gamut mapping ~\cite{zhang2023lookup}.  In general, both $\mathbf{C}$ and ${T}$  are spatially variant and depend on pixel position $\mathbf{x}$.
%Color matching between source and target images has similar form with the linear and non linear parts ~\cite{finlayson2017color} ~\cite{AN1} (more details in suppl. materials).
%We propose 


\begin{figure*}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{fig/main-arch.pdf}
  \vspace{-3mm}
  \caption{a) \textbf{Overview of the cmKAN architecture}, b) Generator Network ($\mathcal{G}$) and its key components: c) Illumination Estimator (IE), d) Color Transformer (CT), and e) Color Feature Modulator (CFM).}
  %\caption{a) \textbf{Overview of the cmKAN architecture.} b) The Generator Network ($\mathcal{G}$) and its main components: c) Illumination Estimator (IE), d) Color Transformer (CT), e) Color Feature Modulator (CFM).}
  \label{fig:overview}
\end{figure*}


\subsection{Generator Network}
\label{sec:generator}
As illustrated in Fig.~\ref{fig:overview} (b), the proposed generator architecture has been designed to efficiently generate 2D coefficient maps for modulating the KAN parameters, while systematically capturing the spatial information critical to KANs. Below, we briefly describe the functionality and contributions of its three specialized modules to the overall process. %This functionality of the generator 
%is achieved via three specialized modules: the Illumination Estimator (IE) responsible for analyzing the illumination component of the input image, the Colour Transformer (CT), which facilitates and refines the color transformations; and the Color Feature Modulator (CFM), which modulates the incoming color information from IE and CT blocks to generate the set of refined parameter maps. Below, we briefly describe the functionality and contributions of each module to the overall process.
%The generator consists of an Illumination Estimator (IE), two Color Transformer (CT) blocks, and a Convex Hull Analyzer (CHA) (fig.~\ref{fig:overview}a,b,c). We also used down-sampling discrete wavelet transform (DWT)~\cite{} blocks to better handle boundaries and low-frequency features. While we designed the generator design, we also focused on its lightweight and efficiency.

\begin{figure}
  \centering
  \includegraphics[width=0.8\linewidth]{fig/ie-ca-arch.pdf}
  \vspace{-2mm}
  \caption{The proposed \textbf{Multi-Scale Color Attention (MCA)} to efficiently exploit the channel-wise dependencies.}
  \label{fig:mca}
\end{figure}


\subsubsection{Illumination Estimator}
\label{sec:IE}
\vspace{-1mm}
 The illumination estimator (Fig.~\ref{fig:overview} (c)) in the generator provides a foundation step for the overall color processing of the input image, $X$. This is crucial because proper illumination correction prevents over-saturation or washed-out colors during color mapping, preserving the scene's natural appearance. By accurately estimating the illumination map, the framework facilitates precise brightness adjustments, ensuring consistent and realistic color reproduction. 
 
In a nutshell, the illumination estimator is a small CNN that processes the input image $X$ and its channel-averaged counterpart $X_{avg}$ to generate an illumination feature $F_i$ and illumination map $M_i$. The module begins by applying a $1\times1$ convolution to the concatenated $X$ and $X_{avg}$, thus effectively integrating the spatial and channel-level information. Next, a $3\times3$ dilated depth-wise convolution with a dilation factor of 2 expands the receptive field, allowing the estimator to incorporate semantic context, particularly for handling over- or under-exposed regions. Finally, another $1\times1$ convolution constructs the illumination map $M_i$ from the feature  representation $F_i$. This generated illumination and features maps guide the multi-scale color attention (MCA) in the subsequent color transformer block for refining the hidden representations. This step ensures improved illumination equalization across the scene and prevents over- or under-exposed areas.
%The architecture is shown in Fig.~\ref{fig:ie-and-mca}a. This block allows the initial normalization of the image. According to the Retinex theory image can be decomposed into two components: $I = R\cdot L$, where $R$ is reflectance and $L$ illumination maps. This Retinex model assumes $I$ is a constant which is not true because different ISPs may estimate illumination in different ways. In this case, this difference in illumination assessment should be taken into account when processing image channels. To highlight the difference in illumination estimates we use the Illumination Estimator, a small CNN that can be represented as $F_i,M_i = \mathcal{E}(X, X_m)$, where $\mathcal{E}$ denotes the illumination estimator, $X$ - input image, $X_m$ averaged channel of $X$, $F_i\in \mathbb{R}^{C\times H\times W}$ denotes illumination feature, and $M_i\in \mathbb{R}^{3\times H\times W}$ denotes illumination map. In the beginning, we apply $1\times 1$ convolution to fuse $X$ and $X_m$. Then we apply $3\times 3$ dilated depth-wise convolution with the factor of 2, to increase the receptive field, because semantic contextual information can be important for processing over- or under-exposed regions. Finally, we again apply $1\times 1$ convolution to build the illumination map from the feature. We use the illumination map and illumination feature as a normalizing trend to initially correct the input image and hidden coefficient representations in the MSA block of the color transformer. These corrections are designed to improve illumination equalization in scenes and to avoid over- or under-lighted areas.
\subsubsection{Color Transformer}
\label{sec:CT}
\vspace{-1mm}
The Color Transformer (CT) block works in close conjunction with the Illumination Estimator (IE) to achieve the color balance and enhance the spatial coherence.
As shown in Fig.~\ref{fig:overview} (d), %c CT adopts a two-scale encoder-like architecture.
 CT block incorporates a ViT-inspired architecture and processes a down-sampled input obtained via the Discrete Wavelet Transform (DWT), which effectively preserves boundary details and low-frequency features. The normalized down-sampled input along with the illumination features are then processed by the proposed Multi-Scale Color Attention (MCA) for enhanced refinement. The generated normalized output from MCA is then subsequently directed to the FFN layer \cite{mst++}, which emphasizes augmenting the features by embedding rich contextual information into the representation.
%The input is downsampled via DWT pre-normalized image which is through the transformer layer. The transformer is a ViT-like block that contains the standard normalization layers (LN), light FFN from MST++ article~\cite{mst++} and our novel Multi-Scale Color Attention (MCA) which takes normalized input signal $X$ and feature $F_i$ generated by Illumination Estimator. 

\noindent\textbf{Multi-Scale Color Attention:}
The proposed Multi-Scale Color Attention (MCA), shown in Fig.~\ref{fig:mca}, builds on RawFormer \cite{perevozchikov2024rawformer} with essential enhancements for improved efficiency. While RawFormer computes similarity between spatially compressed query ($\mathbf{Q}$) and key ($\mathbf{K}$) vectors, MCA applies spatial compression to both using strided convolutions (stride $s=2$) and introduces anchors ($\mathbf{A}$) as intermediaries, which are compressed along the spatial and channel dimensions via strided depthwise separable convolutions. These anchors enable efficient similarity comparison, significantly reducing computational cost without compromising accuracy.
%The proposed Multi-Scale Color Attention (MCA) as shown in Fig.~\ref{fig:mca}, builds on RawFormer \cite{perevozchikov2024rawformer}, but introduces key changes for improved efficiency. RawFormer computes similarity between spatially compressed query ($\mathbf{Q}$) and key ($\mathbf{K}$) vectors, whereas the proposed MCA introduces a more efficient mechanism by applying spatial compression to both query and key vectors using strided convolutions (stride $s=2$). It further incorporates anchors ($\mathbf{A}$), compressed along both the spatial and channel dimensions using strided depthwise separable convolutions, as intermediaries. As shown, these anchors are then used for similarity comparison, significantly reducing the computational cost while preserving the effectiveness of the similarity computation. 
%Unlike RawFormer's direct similarity computation between query ($\mathbf{Q}$) and key ($\mathbf{K}$) vectors, the proposed MCA employs their spatial compression using strided convolutions with a stride of $s=2$ and introduces anchors ($\mathbf{A}$), compressed both spatially with a factor of $s=2$ and channel-wise (factor of $r=2$) via strided and depthwise separable convolutions, as intermediaries for similarity computations. This method significantly reduces the computational overhead of self-attention operations. 
This spatial/channel-wise compression does not affect the global color distributions, but significantly increases the computational efficiency (\textit{More details in Supplementary}). Additionally following \cite{zamir2022restormer}, MCA shifts self-attention from the spatial domain to the channel dimension, thus computing the cross-channel covariance to further encode the global context more efficiently. These modifications enable MCA to retain global modeling capacity for color reconstruction, while significantly reducing complexity. The overall operation of MCA block can be summarised as:
%In Rawformer work~\cite{perevozchikov2024rawformer}, the authors presented a Condensed Query Attention Block, with the main idea of KQV self-attention modification by adding an additional compressed Q vector. This novelty reduced the number of computations by reducing the dimensionality of matrices and maintained both visual quality and semantic consistency, which is critical for unpaired learning. On the other hand, in hyperspectral reconstruction tasks, in MST++ work \cite{mst++} the authors proposed a channel-wise self-attention that showed a good performance due to its ability to learn long channel sequences. However, the potential of these methods was not disclosed. In our work, we combine the approaches of channel-wise self-attention mechanisms and the Q vector compression mechanism. Network Structure is shown in Fig.~\ref{fig:ie-and-mca}b. Firstly, we find a $V$ vector using linear projection and spatially compress $K$ and $Q$ vectors using $3\times3$ convolution for the keys to obtain general information about the image and the query using $3\times3$ DW convolution to focus on spatial structure. The compression does not affect global color distributions but significantly increases computational efficiency Then we calculate anchor information using a combination of DW and PW convolutions. The anchor vector accumulates information on key areas and channel features of the image. We can consider it as a pruned basis for the attention mechanism to build connections between previous layers with fewer channels and the current layer. Secondly, to achieve more computational efficiency, attention is applied horizontally and vertically. The CQA block operation is defined as:

\begin{equation}
\begin{array}{c}
    MCA(\textbf{M}_h, \textbf{M}_v, \textbf{V}) = \textbf{M}_h\cdot(\textbf{M}_v\cdot F_i\textbf{V})\\
    \textbf{M}_h = Softmax(\frac{\textbf{Q}\textbf{A}^T}{t_h}), \textbf{M}_v = Softmax(\frac{\textbf{A}\textbf{K}^T}{t_v})\\
\end{array}
\label{eq:mca}
\end{equation}
where $\textbf{M}_h$ and $\textbf{M}_v$ are horizontal and vertical attention maps obtained via anchor-query pair, and anchor-key pair, respectively; $t_h$,$t_v$ denotes their temperatures; $F_i$ is illumination feature provided by the estimator. It is to be noted that to avoid dimension mismatch when multiplying $\textbf{V}$ by $F_i$, the $F_i$ vector is passed through an strided convolution layer.

\subsubsection{Color Feature Modulator}
\label{sec:CFM}
\vspace{-2mm}
 As shown in Fig.~\ref{fig:overview} (b and e), the proposed Color Feature Modulator (CFM) module processes the concatenated 2D maps ($X'$) from various parts of the generator network. This composite 2D vector, containing multi-scale color-dependent information requires further modulation to generate the set of parameter maps, \( W \)  for the KAN. Thus, for the modulation of $X'$, we first apply linear projections of trainable bias vectors, $B$, to refine the normalized concatenated maps, $X''$. The modulation process is mathematically defined as:  $X_m=B_i\cdot ReLU(X''\cdot B_j)$, where $X''$ represents the normalized input signal, $B_i$, $B_j$ are linear projections of the trainable bias $B$, and $X_m$ represents the output modulated signal. %Notably, the dimensionality of the bias is greater than the number of channels in the modulated signal, $dim(B) > dim(X')$, ensuring a richer representation. (we can mention it in supp)
Finally, the parameter maps, \( W \), are obtained by applying a Feed-Forward Network (FFN) \cite{mst++} as an output projection to further align and refine the modulated signal, $X_m$. This step optimizes the parameter maps for subsequent use in the KAN, enhancing the efficiency and precision of the overall pipeline.
%The final parameter maps are generated after applying the FFN as an output projection to align the output signal. %Before the parameters are fed into the KAN Layer we use a channel-by-channel concatenation of the generated 2d maps from different levels of the generator (Fig.~\ref{fig:overview}). Such a composite vector requires additional refinement. Therefore, output 2D maps have to be modulated to improve the quality of the image translation conducted by KAN layer. To modulate the output signal, we use a Parameter Modulator (PM) based on the attention mechanism (Fig.~\ref{fig:overview} (d)). The modulation process can be written by the following equation: $X_m=B_i\cdot ReLU(X\cdot B_j)$, where $X$ is the input signal, $X_m$ is the output modulated signal, $B_i$, $B_j$ are linear projections of the trainable bias $B$. The size of the bias is larger than the number of channels of modulated signal, $dim(B) > dim(X)$. Finally, we apply the FFN as an output projection to align the output signal.

\subsection{Color Matching Using KAN}
\label{sec:kan}

%\subsection{Spatially parametrized KAN for Color Matching}
%\label{sec:cmKAN_idea}
%According to a several works ~\cite{AN1}, ~\cite{AN9} rendering of the source and target image by different camera ISPs from linear sensor response colors $ {I}_{lin} $ in standard device-independent color space, e.g. XYZ ~\cite{AN3} can be formulated as:
%\begin{equation}\label{eqISP}
%{I}_{rdr}=T(w(\mathbf{x}))({I}_{in}\mathbf{C(\mathbf{x})}).
%\end{equation}
%Where matrix $\mathbf{C}$ represents linear part of the ISP pipeline, including white balancing and of color correction matrix, nonlinear transform ${T}$ implements nonlinear part like tone mapping and gamut mapping ~\cite{zhang2023lookup}.  In general, both $\mathbf{C}$ and ${T}$  are spatially variant and depend on pixel position $\mathbf{x}$.
The color matching process maps the color distribution of a source image to a target image through spatially varying linear and non-linear transformations~\cite{finlayson2017color, AN1}. Traditional methods using CNNs or MLPs approximate these transformations with piecewise linear functions but require deeper architectures for precision, thus increasing the complexity ~\cite{AN3, AN1}. % and often underperforming against classical techniques~\cite{AN3, AN1}. 
KANs can address this issue by leveraging Kolmogorov's approximation theorem~\cite{kolmogorov:superposition}, efficiently capturing non-linearities with minimal network depth. Using adaptive spline-based activation functions, KANs can precisely model complex transformations, such as color homography or non-linear tone mapping, outperforming traditional networks reliant on fixed activations, such as ReLU or sigmoid~\cite{AN6}.


%The color matching process involves mapping the color distribution of a source image to that of a target image through spatially varying linear and nonlinear transformations~\cite{finlayson2017color, AN1}. Traditional convolutional neural networks (CNNs) or multilayer perceptrons (MLPs) \cite{}, approximate these transformations using piecewise linear functions.
%However, their reliance on deeper architectures to achieve precision increases computational complexity and consequently they often underperforms compared to classical approaches~\cite{AN3, AN1}. Kolmogorov-Arnold Networks (KANs) provide a more efficient alternative by leveraging Kolmogorov's approximation theorem~\cite{kolmogorov
%}. They excel in capturing the inherent nonlinearities of color matching tasks without requiring excessive network depth, ensuring computational efficiency and superior accuracy~\cite{AN6}.  Using spline-based activation functions-flexible and precise b-splines, KANs adaptively model complex transformations, including those introduced by color homography or localized nonlinear tone mapping. This adaptability allows KANs to effectively and efficiently align the source and target color spaces, outperforming traditional networks reliant on fixed activation functions like ReLU or sigmoid.

% latest one to comment As stated earlier, the process of color matching involves mapping the color distribution of a source image to that of a target image through spatially varying linear and nonlinear transformations~\cite{finlayson2017color, AN1}. Traditional convolutional neural networks (CNNs) or multilayer perceptrons (MLPs), attempt to approximate these transformations using piecewise linear functions. However, their reliance on such approximations often demands deeper networks, significantly increasing computational complexity while still falling short in performance compared to classical methods~\cite{AN3, AN1}. Kolmogorov-Arnold Networks (KANs) offer a promising alternative by addressing these limitations through their ability to approximate smooth functions with high fidelity and efficiency~\cite{AN6}. 

%Color matching between source and target images has similar form with the linear and non-linear parts ~\cite{finlayson2017color} ~\cite{AN1} (more details in suppl. materials) so it needs approximation of smooth nonlinear functions.
%In contrast, traditional convolutional neural networks (CNNs) or multilayer perceptrons (MLPs) construct piecewise linear functions, necessitating a significant increase in the number of layers to achieve satisfactory performance. Recent works on color correction ~\cite{AN3} and color matching ~\cite{AN1} tell us that classical methods still outperform neural one. An alternative approach involves the use of Kolmogorov-Arnold Networks (KANs), a relatively novel neural network architecture that has shown promise in approximating smooth functions with high accuracy and efficiency ~\cite{AN6}. 

%Color matching tasks often involve the approximation of smooth functions, as the image signal processing (ISP) pipeline typically combines nonlinear tone and gamut mapping with linear reduction of color coordinates, considering white point (WP) and spectral sensitivities of the sensor.  

%In contrast, traditional convolutional neural networks (CNNs) or multilayer perceptrons (MLPs) construct piecewise linear functions, necessitating a significant increase in the number of layers to achieve satisfactory performance. An alternative approach involves the use of Kolmogorov-Arnold Networks (KANs), a relatively novel neural network architecture that has shown promise in approximating smooth functions with high accuracy and efficiency. 

%latest one to comment Unlike conventional architectures, KANs are specifically designed to capture the non-linearities inherent in color matching tasks without the need for excessive depth, making them computationally efficient and highly accurate. This capability is rooted in Kolmogorov's approximation theorem~\cite{kolmogorov:superposition}, which forms the theoretical foundation for KANs. By leveraging spline-based activation functions — piecewise polynomials capable of flexible and precise approximations, KANs surpass the limitations of traditional networks that rely on fixed activation functions such as ReLU or sigmoid. These b-spline functions provide a smooth and adaptive mechanism to model the complex transformations often encountered in color matching, such as the unknown curves introduced by color homography effects or localized nonlinear tone mapping. As a result, KANs effectively approximate these intricate relationships, enabling robust and accurate alignment of source and target color spaces. 
%KANs are grounded in Kolmogorov's approximation theorem ~\cite{kolmogorov:superposition} and leverage the power of spline-based activation functions, which are piecewise polynomials that enable more nuanced and flexible approximations of complex functions. Unlike traditional neural networks that rely on fixed activation functions like ReLU or sigmoid, KANs utilize these b-spline functions. In addition, spline gives a smooth approximation to unknown curves that may appear due to color homography effects and as a consequence of local nonlinear tone mapping. In this work we use only one KAN(3,3) layer~\cite{AN6} to adjust the colors:
In our cmKAN, we employ a single KAN (3,3) layer~\cite{AN6} to adjust the colors, formulated as:
%\begin{equation}\label{eq:KAN}
%\hat{t}_j = \sum_{i=1}^{3} \left(u_{ij} silu(s_i) + v_{ij} \sum_{m=0}^{G+k-1} c_{ijm} B_{ijm}(s_i)\right).
%\end{equation}

\begin{equation}\label{eq:KAN}
\hat{y}_j = \sum_{i=0}^{2} \left(u_{ij} silu(x_i) + v_{ij} \sum_{m=0}^{G+k-1} c_{ijm} B_{ijm}(x_i)\right)
\end{equation}

\noindent where, ${x_i}$, ${\hat{y}_j}$ represents the input and output components of the RGB color space, respectively. Here, ${silu(.)}$ is residual activation function, $B_{ijm}(.)$ are the b-spline basis functions, 
%of the spline $ij$ that approximate the smooth functions described in Kolmogorov's theorem, 
and $u_{ij}$, $v_{ij}$, $c_{ijm}$ are KAN layer non-trainable parameters which are obtained from the generator's output via channel splitting: $W=(W_u,W_v,W_c)$. \textit{(More mathematical details are in Supp.)} Every point $(a,b)$ of generator's output $W$ represents set of KAN  parameters: $u_{ij}=W_u(a,b)_{ij}$, $v_{ij}=W_v(a,b)_{ij}$, $c_{ij}=W_c(a,b)_{ij}$. 


%where, ${x_i}$, ${\hat{y}_j}$ represents the input and output components of the RGB color space, respectively. Here, ${silu(.)}$ is residual activation function, $B_{ijm}(.)$ are the b-spline basis functions of the spline $ij$ that approximate the smooth functions described in Kolmogorov's theorem, and $u_{ij}$, $v_{ij}$, $c_{ijm}$ are KAN layer non-trainable parameters provided by our generator $\mathcal{G}$ that collaboratively define how the input is transformed. 


%Each super-pixel in 
%Every point $(a,b)$ of generator's output $W$ represents 1D vector of KAN  parameters in (\ref{eq:KAN})":

%\begin{equation}\label{eq:KAN-supstitution}
%\begin{array}{c}
%    w=\{u_{ij}, v_{ij}, c_{ijm}\}; w(x,y)\in W\\
%    i=0..2, j=0..2,m=0..G+k-1,\\
%\end{array}
%\end{equation}
%\begin{equation}\label{eq:KAN-supstitution}
%\begin{array}{c}
%\mathcal{G}(X,\theta)= W(a,b)=\{u_{ij}, v_{ij}, c_{ijm}\};\\
 %   \mathcal{G}(X,\theta)=W(a,b);\\
  %  i=0..2, j=0..2,m=0..G+k-1,\\
%\end{array}
%\end{equation}
%where $G$ and  $k$ represents the spline grid size, and the spline order, respectively, and $X$ is input image.

%where ${s_i}$, ${\hat{t}_i}$ input and output component of RGB color, ${silu(x)}$ is residual activation function, $B_{ijm}(s_i)$ are b-spline basis functions of the spline $ij$ , $G$ is spline grid size,  $k $ is spline order, $c_{ijm}$ is spline parameters, $u_{ij}$ and $v_{ij}$ are additional parameters of the residual activation. 

%Parameters $c_{ijm}$, $u_{ij}$  and $v_{ij}$ form KAN parameters vector $w=\{c_{ijm}, u_{ij}, v_{ij}\}$, and as we can see from the (\ref{eq:KAN}) this vector is global for the image, while it can include areas with different color rendering e.g. due to spatially dependent tone-mapping or gamut-mapping. To fuse the power of spline with spatial information we perform the parameter substitution from our generator network (Fig. \ref{fig:overview}). %Therefore, the full image translation function can be defined as:
%\begin{equation}\label{eq:KAN-full}
%\hat{y} = KAN(\mathcal{G}(x,\theta),x),
%\end{equation}
%where $KAN$ represents KAN Layer (Eq. \ref{eq:KAN}), $\mathcal{G}$ is our generator with $\theta$ trainable parameters, $x,y$ input and output images. %For our experiments, we use spline with the order $k=3$ and grid size $G=5$. That's why we have to generate a 2D map with 90 channels.

For our experiments, we utilize a spline of order $k=3$, with a grid size $G=5$, resulting in the generation of a 2D map with 90 channels. This setup ensures that the generated parameter maps are sufficiently expressive to capture local variations in color matching, enabling precise and spatially coherent transformations across the entire image. By integrating the generator's role as a hypernetwork for dynamically generating weights with KAN's smooth approximation capabilities, the proposed framework achieves robust and efficient color adjustment. This synergy enables precise spatial adaptivity while maintaining computational efficiency, allowing the full color-matching function to be formally defined as:
\begin{equation}\label{eq:KAN-full}
\hat{Y} = KAN(\mathcal{G}(X,\theta),X),
\end{equation}
where, $KAN$ represents the KAN layer (Eq. \ref{eq:KAN}), $\mathcal{G}$ is our generator with $\theta$ trainable parameters, and $X,\hat{Y}$ represents the input and output images, respectively. Next, we discuss how the model is adapted for supervised, unsupervised, and paired-based optimization scenarios.
%KANs are grounded in Kolmogorov's approximation theorem, which is mathematically expressed as:

%\begin{equation}
%f(x_1, \dots, x_n) = \sum_{m=1}^{2n+1} \phi_m \left( \sum_{j=1}^n \psi_{m,j}(x_j) \right)
%\end{equation}

%This theorem asserts that any multivariate function can be exactly represented by a composition of univariate functions and addition. KANs generalize the Kolmogorov-Arnold representation to arbitrary widths and depths.

%TODO: Write the process of substitution of parameters. Taking into account theorem X we can write an equation of the KAN layer. This layer has P learnable parameters. The main limitation of KAN-s that they can't accumulate spatial information by design. That's why we decided to generate it's parameters using our encoder. Although there are early works with KAN Convolution Layer implementations, the use of such blocks is associated with high computational costs. Therefore, we propose an innovative approach to generating spline coefficients using traditional methods. This can significantly reduce computational costs. For greater efficiency, we use one KAN layer (3,3) since we have mathematical proof of the sufficiency of using one layer for color matching tasks. This evidence is given in the supplementary materials.


\subsection{Supervised Learning}
\label{sec:supervised}
Let \( X \) and \( Y \) represent an input image and its corresponding target image, respectively. For the supervised learning approach, the proposed  cmKAN model generates an estimated image \( \hat{Y} \) from \( X \), aiming to approximate the color characteristics of the target image \( Y \) (Eq.~\ref{eq:KAN-full}). 
%Denote by x and y an input image and the corresponding target image. Our cmKAN are used to produce an image $\hat{y}$ from x for approximating the color characteristic of target image y,
% \begin{equation}
% \hat{Y} = cmKAN(X,\theta) 
% \end{equation}
% where $\theta$  represents it's trainable parameters. 
The overall framework is trained using the following loss function:
\begin{equation}\label{eq:pix-wise}
\mathcal{L}_{pixel-wise}(Y,\hat{Y}) = \ell_{1} + \beta_0 (1-SSIM)
\end{equation}
where $\beta_0=0.15$, and $\ell_{1}$ and $SSIM$ refer to L1 loss and the structural similarity index measure (SSIM) \cite{wang2004image}, respectively. %We use the Adam optimizer with betas set to (0.9, 0.99), a learning rate of 0.001, and a weight decay of 0.05 for 450 epochs. The learning schedule was managed using the cosine annealing warm restarts strategy~\cite{}.

\subsection{Unsupervised Learning}
\label{sec:unsupervised}
In our unsupervised learning approach, we adopted two-stage training strategy: (1) generator pre-training and (2) unpaired image-to-image training using a CycleGAN-like framework~\cite{zhu2017unpaired}. For network's pretraining, the input images were divided into $32 \times 32$ patches, and a color transformation including random jitter in the range (-30\%, +30\%) of brightness, contrast, saturation, hue, color shift, and random channel reordering were randomly applied to each patch with 60\% coverage of the image. The overall objective of the generator in  pre-training stage was to reconstruct the original image colors from these partially altered patches via minimizing the pixel-wise loss function in Eq.~\ref{eq:pix-wise}.

%For unsupervised learning, we used a rawformer-like training approach, which includes two stages: generator pre-training and image-to-image unpaired training using CycleGAN-like approach~\cite{}. 

%Inspired by the effective technique of the generator pre-training, we also apply pre-training for our cmKAN block. Since our block only processes colors and cannot solve the inpainting problem, for this stage, we are trying to solve the color reconstruction problem. The input image was divided into patches of size $32\times32$ and a color transformation including random jitter in the range of (-30\%...+30\%) of brightness, contrast, saturation, hue, color shift, and random channel reordering was randomly applied to each patch with 60\% coverage of the image.
%The objective of the generator during this stage was to reconstruct the original colors of the image from its partially obscured version. The training was performed using the AdamW optimizer~\cite{} with betas set to (0.9, 0.99) and a weight decay of 0.05 for 200 epochs to minimize the pixel-wise loss function~\ref{eq:pix-wise}
Following pre-training, unpaired color matching was performed to jointly train our cmKAN and a discriminator network. Here, we use the discriminator network proposed in \cite{perevozchikov2024rawformer}. 
%Thereafter, we started our unpaired raw-to-raw translation task for an additional 500 epochs, while simultaneously training the discriminator networks. We use the Adam optimizer~\cite{} with betas set to (0.5, 0.99) and a learning rate of 0.0001 for the discriminator networks and
%0.00005 for the generator networks.
% TEXT COPIED FROM RAWFORMER PAPER
During this stage, the discriminator networks were optimized to minimize the following loss functions:

\begin{equation}
\label{eq:disc1}
    \mathcal{L}^{dis}_A = \ell_{gan}(D_A(G_{B \rightarrow A}(b)), 0) + \ell_{gan}(D_A(a), 1)
\end{equation}
\begin{equation}
\label{eq:disc2}
    \mathcal{L}^{dis}_B =  \ell_{gan}(D_B(G_{A \rightarrow B}(a)), 0) +  \ell_{gan}(D_B(b), 1)
\end{equation}

\noindent where $a$ and $b$ represent images from the source and target color distributions $A$ and $B$, respectively, while $G_{B \rightarrow A}(b)$ and $G_{A \rightarrow B}(a)$ are the output images produced by each generator network, respectively. The labels $0$ and $1$ represent ``fake'' and ``real'' images, respectively, and $\ell_{gan}(\cdot)$ computes the cross-entropy loss. 

The weights of two cmKAN models -- one mapping from source to target and the other from target to source color distributions -- were optimized to minimize the following loss function:

{\scriptsize\begin{equation}
    \mathcal{L}^{gen} = \beta_1(\mathcal{L}^{gan}_A + \mathcal{L}^{gan}_B) + \beta_2(\mathcal{L}^{idt}_A + \mathcal{L}^{idt}_B) + \beta_3(\mathcal{L}^{cyc}_A + \mathcal{L}^{cyc}_B)
    \label{eq:gen1}
\end{equation}}

\noindent where $\beta_1$, $\beta_2$, and $\beta_3$ where set to 1, 10, 0.5, respectively; $\mathcal{L}^{gan}_A$ and $\mathcal{L}^{idt}_A$  refer to $\ell_{gan}(D_B(G_{A \rightarrow B}(a)), 1)$ and $\mathcal{L}_{pixel-wise}(G_{B \rightarrow A}(a), a)$, respectively. $\mathcal{L}^{cyc}_A$ is $\mathcal{L}_{pixel-wise}( G_{B \rightarrow A}(G_{A \rightarrow B}(a)), a)$. Note that at inference time, only a single cmKAN (e.g., $G_{A \rightarrow B}$) is required to map colors from the source color distribution (e.g., $A$) to the target color distribution (e.g., $B$).



\subsection{Paired-Based Optimization}
\label{sec:optimization}

For paired-based optimization, we used pairs of corresponding colors for the source and target images  to align their color distributions effectively. For training between image pairs, we employed cmKAN-Light, a lightweight variant of our full model, optimized for faster performance. 
 Unlike the original architecture depicted in Fig.~\ref{fig:overview}, cmKAN-Light is simplified to include only a single Color Transformer (CT) block and one Discrete Wavelet Transform (DWT) block, reducing computational complexity while maintaining essential functionality. 
 Given the need for efficient online optimization, we adopted a two-stage approach. First, to provide a robust initialization, we pre-trained the cmKAN-Light model on the corresponding dataset using the supervised learning approach outlined in (Sec.~\ref{sec:supervised}). This step generated a set of well-initialized parameters, serving as a starting point for fine-tuning. Subsequently, fine-tuning was performed directly on the particular image pairs, allowing the model to adapt to specific pairwise relationships.
 To further accelerate training, we employed an L1 loss function over just 10 iterations, ensuring rapid convergence. This strategy enables cmKAN-Light to achieve effective color matching with minimal computational overhead, making it well-suited for online optimization tasks.
 
 
 %Since the speed of optimization is important in online optimization we used a starting point for parameter initialization. To get initialized weights, we pre-trained our cmKAN-Light once on the corresponding dataset using our previously described supervised learning approach (Sec.~\ref{sec:supervised}). Then we performed fine-tuning of the trained model on the particular image pair. To increase the training speed we used only L1 loss for 10 iterations.




%Typical number of such color-pairs for our dataset is about 15K. In the case of the SMS pipeline we utilized Differential Evolution for constrained global optimization, for the paired color stabilization using pure KAN model we used Adam optimizer with betas $= (0.9, 0.999)$, learning rate $= 0.01$ and batch size of 4096. Training for simple KAN model from scratch takes 10K iterations. To speed it up, we treated each image pair as separate domain, and apply model agnostic meta-learning approach from \cite{soh2020meta} to obtain more appropriate starting checkpoint, which allows to reduce number of training iterations to 300.






==> sec/4_results.tex <==

\section{Experiments}
\label{sec:experiments}

In this section, we evaluate our cmKAN across a range of color-matching tasks in different scenarios, including supervised, unsupervised, and paired-based optimization. First, we evaluate our method on unsupervised raw-to-raw mapping, where the goal is to map raw images from a source camera to the raw color space of a target camera. Next, we apply our approach to supervised raw-to-sRGB mapping, where our network learns the ISP non-linear color mapping function. Finally, we evaluate cmKAN on sRGB-to-sRGB mapping, to transfer colors from a source color distribution to a target distribution, such as professional photographer edits \cite{AN7} or another camera ISP rendering \cite{AN2}. Additionally, we test our method on our proposed dataset of paired sRGB images rendered by the camera ISP and captured by two different cameras. For this sRGB-to-sRGB mapping task, we present results across the three scenarios: unsupervised, supervised, and paired-based optimization.


\subsection{Datasets}
We begin by introducing our dataset, collected to support the training and evaluation of sRGB-to-sRGB mapping for images captured by two different cameras. Next, we provide an overview of the datasets used throughout our evaluation, organized by each specific task.
%\vspace{-5mm} %shrink!
\subsubsection{Proposed dataset}
\label{sec:proposed-datset}
To validate our cross-camera mapping in sRGB color space, we collected a dataset of 2,520 sRGB images captured by the wide and main cameras (1,260 images per camera) of the Huawei P40 Pro smartphone. These cameras use distinct sensor types: a Quad-Bayer RGGB (Sony IMX700) for the wide camera and an RYYB (Sony IMX608) for the main camera. We used the on-device camera ISP to render images to the sRGB space. sRGB image pairs were then spatially aligned by first identifying keypoints with the SURF detector \cite{bay2006surf} and matching features using the KNN algorithm with Lowe's ratio test \cite{lowe2004distinctive}. A projective transformation matrix was subsequently applied to warp the images. Since both cameras are fixed within the smartphone, this stable positioning helped to significantly minimize misalignment errors. Finally, all aligned images were manually reviewed to discard any remaining misaligned pairs. Our dataset reflects real-world conditions, with images captured under diverse lighting and seasonal variations \textit{(see supp. materials for additional details).}


\subsubsection{Raw-to-raw mapping}
For this task, we utilized the raw-to-raw mapping dataset \cite{afifi2021semi}, which contains a total of 392 unpaired raw images (196 from each of the Samsung Galaxy S9 and iPhone X). Additionally, the dataset includes 115 paired testing raw images from each camera for evaluation.

\subsubsection{Raw-to-sRGB mapping}
For this task, we utilized the Zurich raw-to-sRGB dataset~\cite{ignatov2020replacing} to evaluate our method on the raw-to-sRGB task. This dataset consists of 48,043 paired raw images and their corresponding sRGB-rendered outputs, captured simultaneously with a Huawei P20 smartphone camera and a Canon 5D Mark IV DSLR camera. For our experiments, we used 70\% of the images for training and 30\% for testing.


\subsubsection{sRGB-to-sRGB mapping}

As mentioned previously, in the sRGB-to-sRGB task, we apply color matching to emulate specific photographer styles, replicate the color rendering of target camera ISPs, and align colors between sRGB images captured by two different cameras within a dual-camera device. For the photographer-style matching, we used the MIT-Adobe FiveK dataset \cite{AN7}, which provides expert-adjusted ground-truth styles. We specifically chose expert style C as our target, as it is widely referenced in prior work \cite{chen2018deep, wang2019underexposed, afifi2021learning}. In our experiments, we employed 5K images for supervised training and 498 images for evaluation. 
%Additionally, we examined the PPR10K dataset \cite{AN8}, which consists of 10K raw images rendered by three different expert photographers. For this dataset, we used 7K images for supervised training and 3K images for evaluation.

For camera rendering mapping, we conducted paired-based optimization evaluations using the dataset from \cite{AN2}, which includes 35 images captured by two DSLR cameras (Nikon D3100 and Canon EOS 80D) from the same scenes with slightly different camera positions. This dataset provides synthetic ground-truth images to support color rendering transfer from the source to the target camera, ensuring well-aligned ground-truth pairs.


Finally, we used our proposed  dual-camera sRGB dataset to evaluate all the three scenarios: supervised, unsupervised, and paired-based. For both the supervised and unsupervised experiments, 900 images were allocated for training and 350 images for testing.

% \begin{table}[h]
%   \centering
%   \resizebox{\linewidth}{!}
%   {
%   \begin{tabular}{@{}l|r|l|r@{}}
%     \toprule
%     Scene class        & Count & Image class & Count  \\
%     \midrule
%     Indoor            & 114 & City & 324 \\
%     Outdoor/spring    & 109 & Countryside & 164 \\
%     Outdoor/summer    & 558 & Forest & 49 \\
%     Outdoor/autumn    & 175 & Mountains & 166 \\
%     Outdoor/winter    & 97 & Seaside & 161 \\
%     Low-light       & 107 & Sunset & 92 \\
%     \textbf{Total}    & 1260 & Difficult illumination & 21 \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Scene and image classes in our dataset.}
%   \label{tab:our-dataset}
% \end{table}




% TODO - write the text about Javier's data, raw-to-RGB datasets (ZRR, AIM, S7), and raw-to-raw datasets.

% \textbf{A Real-World Dataset:} 
% TODO - write the text about our dataset

\subsection{Training details}
We used the following patch sizes for training: 256$\times$256 patches for raw-to-raw mapping, 448$\times$448 patches for raw-to-sRGB, and 1024$\times$1024 patches for sRGB-to-sRGB mapping. In all the experiments, we used Adam optimizer~\cite{kingma2014adam} for supervised training, unsupervised training, and paired-based optimization with betas set to (0.9, 0.99).

For unsupervised training, we first trained our cmKAN on the color reconstruction task (as explained in Sec.~\ref{sec:unsupervised}) for 200 epochs, and then trained it on the unpaired data for the color-matching task for an additional 500 epochs. We used a learning rate of 0.0001 for the discriminator networks to minimize Eqs.~\ref{eq:disc1} and \ref{eq:disc2}, and a learning rate of 0.001 for the cmKAN models to minimize Eq.~\ref{eq:gen1}.  For supervised training (i.e., raw-to-sRGB and supervised sRGB-to-sRGB), we trained our model for 450 epochs to minimize the loss function in Eq.~\ref{eq:pix-wise}. For both supervised training and paired-based optimization, we used a learning rate of 0.001.

\subsection{Results}




\subsubsection{Raw-to-raw mapping results}

\begin{figure}[t]
  \centering
  %\includegraphics[width=1.\linewidth]{fig/qualtative-result1.pdf}
  \includegraphics[width=0.8\linewidth]{fig/vis-raw.png}
    \vspace{-2mm}
  \caption{
  Qualitative comparison of unsupervised \textit{raw-to-raw mapping} on the
dataset in \cite{afifi2021semi}. Our cmKAN method achieves the most accurate color mapping with lower $\Delta E$ errors, while being more lightweight than RawFormer~\cite{perevozchikov2024rawformer}. Gamma operator is applied to aid visualization. Best viewed in the electronic version.}
  \label{fig:qualtative-raw2raw}
\end{figure}

We compare our unsupervised-trained model for raw-to-raw mapping against the following methods (trained in an unsupervised or semi-supervised manner as described in \cite{perevozchikov2024rawformer} and \cite{afifi2021semi}, respectively): SSRM \cite{afifi2021semi}, UVCGANv2 \cite{torbunov2023uvcgan2}, and RawFormer \cite{perevozchikov2024rawformer}. We report PSNR, SSIM, and $\Delta E$ errors in Table \ref{tab:raw-to-raw} for the raw-to-raw mapping dataset \cite{afifi2021semi}. As shown, our method achieves better or comparable results to the recent work in \cite{perevozchikov2024rawformer}, while being lightweight and more compatible with limited computational resources. Qualitative examples demonstrating the efficacy of the proposed method are shown in  Fig.~\ref{fig:qualtative-raw2raw} \textit{(more in supp. materials).}

\begin{table}[h]
  \centering
    \caption{Results for \textit{unsupervised} raw-to-raw mapping using the dataset in \cite{afifi2021semi}. The best results are highlighted in yellow. \label{tab:raw-to-raw}}
    \vspace{-2mm}
  \resizebox{0.8\linewidth}{!}
  {
  \begin{tabular}{@{}l|ccc|ccc@{}}
    \toprule
    Method & PSNR & SSIM & $\Delta E$ & PSNR & SSIM & $\Delta E$\\
    & \multicolumn{3}{c|}{\colorbox{supervised}{Samsung-to-iPhone}} & \multicolumn{3}{c}{\colorbox{unsipervised}{iPhone-to-Samsung}}\\
    \midrule
    SSRM~\cite{afifi2021semi}    & 29.65 & 0.89 & 6.32 & 28.58 & 0.90 & 6.53 \\
UVCGANv2~\cite{torbunov2023uvcgan2}  & 36.32 & 0.94 & 4.21 & 36.46 & 0.92 & 4.73 \\
    RawFormer~\cite{perevozchikov2024rawformer}& 40.98 & \colorbox{best}{0.97} & 2.09 & \colorbox{best}{41.48} & \colorbox{best}{0.98} & 1.99 \\
    cmKAN     & \colorbox{best}{41.01} & \colorbox{best}{0.97} & \colorbox{best}{1.23} & 41.47 & \colorbox{best}{0.98} & \colorbox{best}{1.27} \\
    \bottomrule
  \end{tabular}
  }  \vspace{-2mm}
  \label{tab:raw}
\end{table}


\subsubsection{Raw-to-sRGB mapping results}

\begin{figure}[t]
  \centering
  %\includegraphics[width=1.\linewidth]{fig/qualtative-result1.pdf}
  \includegraphics[width=0.9\linewidth]{fig/vis-isp.png}
    \vspace{-2mm}
  \caption{Qualitative comparison of raw-to-sRGB rendering on the Zurich raw-to-sRGB dataset~\cite{ignatov2020replacing}. Our cmKAN method achieves the most accurate color mapping with lower $\Delta E$ errors. Best viewed in the electronic version.}
  \vspace{-2mm}
  \label{fig:qualtative-isp}
\end{figure}

We compare our method for learning raw-to-sRGB color rendering in camera ISPs against the following methods (all trained in a supervised manner on the same dataset): %MW-ISP~\cite{ignatov2020aim}, LAN-ISP~\cite{wirzberger2022lan}, DH-ISP~\cite{ignatov2021learned}, and RawFormer~\cite{perevozchikov2024rawformer}
MW-ISP~\cite{ignatov2020aim}, LiteISP~\cite{zhang2021learning}, MicroISP~\cite{ignatov2022microisp} , and SimpleISP~\cite{elezabi2024simple}. Table \ref{tab:isp} reports PSNR, SSIM, and $\Delta E$ error %and reproduction angular error~\cite{finlayson2014reproduction}
metrics demonstrating that our method achieves promising results with reduced computational cost (FLOPs). Qualitative examples are shown in Fig.~\ref{fig:qualtative-isp} \textit{(more in supp. materials)}.

\begin{table}[t]
  \centering
    \caption{Results for \textit{supervised} raw-to-sRGB mapping on the Zurich raw-to-sRGB dataset~\cite{ignatov2020replacing}. }%  Ours is better. Input = (3,1024,1024)}
      \label{tab:isp}
          \vspace{-2mm}
  \resizebox{0.65\linewidth}{!}
  {
  \begin{tabular}{@{}l|ccc|c@{}}
    \toprule
    Method & PSNR & SSIM & $\Delta E$ & FLOPs \\
    \midrule
    MW-ISP~\cite{ignatov2020aim}  & 21.88 &  0.82 & 10.33 &  3.6T\\
    %LAN-ISP~\cite{wirzberger2022lan} & 20.76 & 0.81 & 10.41 & 56.9G\\
    LiteISP~\cite{zhang2021learning} & 22.18 &  0.83 & 10.28 & 174G\\
    MicroISP~\cite{ignatov2022microisp} & 20.30 & 0.78 & 11.14 & \colorbox{best}{37G}\\
    SimpleISP~\cite{elezabi2024simple} & 24.18 & 0.84 & 10.02 & 58G\\
    %RawFormer~\cite{perevozchikov2024rawformer} & 24.34 & \colorbox{best}{0.85} & 9.18 &  2.7T\\
    cmKAN   & \colorbox{best}{24.41} & \colorbox{best}{0.85} &  \colorbox{best}{7.27} & 40G\\
    \bottomrule
  \end{tabular}
  \vspace{-5mm}
  }
\end{table}

\subsubsection{sRGB-to-sRGB mapping results}

\begin{figure*}[t]
  \centering
  %\includegraphics[width=1.\linewidth]{fig/qualtative-result1.pdf}
  \includegraphics[width=0.9\linewidth]{fig/vis-samara.pdf}
  \vspace{-2mm}
  \caption{Qualitative comparison of sRGB-to-sRGB color matching on our dataset. In (a), we show three scenarios using our method: unsupervised learning (green), supervised learning (purple), and paired-based optimization (red). Our method demonstrates superior color matching compared to other methods (UVCGAN v2~\cite{torbunov2023uvcgan2}, Rawformer~\cite{perevozchikov2024rawformer}, SepLUT~\cite{yang2022seplut}, SIRLUT~\cite{li2024sirlut}, NeuralPreset~\cite{ke2023neural}, and Rodriguez \textit{et al}.'s method~\cite{AN2}). %, even under low-light conditions (marked with a moon icon), with the lowest $\Delta E$ errors. 
  In (b), we show results from a single scene across the three scenarios using our method, showcasing consistent color-matching accuracy.}
  \vspace{-3mm}
  \label{fig:qualtative-srgb2srgb}
\end{figure*}

In Table~\ref{tab:cm-ours}, we report the results on our proposed dataset in three different scenarios. Firstly,  we compare our unsupervised-trained model against other unsupervised methods, namely UVCGANv2~\cite{torbunov2023uvcgan2} and RawFormer~\cite{perevozchikov2024rawformer}. Then, we compare our supervised-trained model against several methods trained in a supervised manner, including: %PCE~\cite{chai2020supervised}, 
%NeurOP~\cite{wang2022neural}, AdaInt~\cite{yang2022adaint}, 
SepLUT~\cite{yang2022seplut}, %RetinexFormer~\cite{cai2023retinexformer},
MW-ISP~\cite{ignatov2020aim},
LYT-Net~\cite{brateanu2024lyt}, and SIRLUT~\cite{li2024sirlut}. Lastly, we compare our paired-based optimization results against other paired-based methods for color matching and transfer. Specifically, we compare our results with the following methods: polynomial mapping~\cite{hong2001study}, root-polynomial mapping~\cite{finlayson2015color}, %color homography~\cite{finlayson2017color},
%color-matcher~\cite{plenopticam}, 
NeuralPreset~\cite{ke2023neural}, and Rodriguez et al.'s method~\cite{AN2}. 
%First, we compare our paired-based optimization results against other paired-based methods for color matching and transfer. Specifically, we compare our results with the following methods: polynomial mapping~\cite{hong2001study}, root-polynomial mapping~\cite{finlayson2015color}, %color homography~\cite{finlayson2017color},
%color-matcher~\cite{plenopticam}, 
%NeuralPreset~\cite{ke2023neural}, and Rodriguez et al.'s method~\cite{AN2}. Furthermore, we compare our supervised-trained model against several methods trained in a supervised manner, including: %PCE~\cite{chai2020supervised}, 
%NeurOP~\cite{wang2022neural}, AdaInt~\cite{yang2022adaint}, 
%SepLUT~\cite{yang2022seplut}, %RetinexFormer~\cite{cai2023retinexformer},
%MW-ISP~\cite{ignatov2020aim},
%LYT-Net~\cite{brateanu2024lyt}, and SIRLUT~\cite{li2024sirlut}. Lastly, we compare our unsupervised-trained model against other unsupervised methods, namely UVCGANv2~\cite{torbunov2023uvcgan2} and RawFormer~\cite{perevozchikov2024rawformer}
As shown, our method achieves the best results across all metrics, while requiring less inference time and having fewer parameters compared to the other methods. Qualitative comparisons for the same are shown in Fig.~\ref{fig:qualtative-srgb2srgb} \textit{(more results in supp. materials)}.

Lastly, the results on the MIT-Adobe FiveK~\cite{AN7}  dataset for supervised sRGB-to-sRGB mapping to emulate a specific photographer style, are presented in Table \ref{tab:cm-5k} (\textit{results on the PPR10K dataset~\cite{AN8}
for the same task are in supp. materials}). 

The results clearly show that our method consistently outperforms alternative approaches across various color-matching tasks. Additionally, we validated our results by conducting a user study that shows \textbf{\textit{2x superior MOS scores}} over other methods \textit{(see supp. materials for more details)}.

\begin{table}[t]
  \centering
    \caption{Results of sRGB-to-sRGB mapping on our dataset. We compare the results of \textit{unsupervised} trained models, \textit{supervised} trained models, and \textit{paired-based inference}. Inference times were measured on GPU (except for methods marked by *, which were run on CPU).}
    \vspace{-2mm}
  \label{tab:cm-ours}
  \resizebox{0.9\linewidth}{!}
  {
  \begin{tabular}{@{}l|ccc|cc@{}}
    \toprule
    Method & PSNR & SSIM & $\Delta E$ & \#Params & Time\\
    \midrule
     & \multicolumn{3}{c|}{\colorbox{unsipervised}{Unsupervised training}} & \\
    UVCGANv2~\cite{torbunov2023uvcgan2}& 22.89 & 0.74 & 6.44 & 32.6M & 2.1s\\
    RawFormer~\cite{perevozchikov2024rawformer}& 23.81 & 0.77 & 5.78 & 26.1M & 6.7s\\
    cmKAN  & \colorbox{best}{25.64} &  \colorbox{best}{0.88} &  \colorbox{best}{4.86} &   \colorbox{best}{76.4K} &  \colorbox{best}{1.1s}\\
    \midrule
     & \multicolumn{3}{c|}{\colorbox{supervised}{Supervised training}} & \\
    %DH-ISP~\cite{ignatov2021learned}    & 22.12 & 0.72 & 7.12 & 5.23 & 4.9K & \colorbox{best}{0.5s}\\
    %PCE~\cite{chai2020supervised}           & 22.57 & 0.73 & 6.51 & 4.91 & 1.3M & 4.1s\\
    %NeurOp~\cite{wang2022neural}        & 22.69 & 0.73 & 6.43 & 4.89 & \colorbox{best}{28.7K} & 1.3s\\
    %AdaInt~\cite{yang2022adaint}        & 22.84 & 0.74 & 6.34 & 4.83 & 619.7K & 3.2s\\
    SepLUT~\cite{yang2022seplut}        & 22.86 & 0.74 & 6.31 & 119.8K & 2.1s\\
    MW-ISP~\cite{ignatov2020aim}        & 23.31 & 0.76 & 5.93 & 29.2M & 8.8s\\
    %LAN-ISP~\cite{wirzberger2022lan}       & 23.46 & 0.77 & 5.89 & 4.65 & 49.2K & 1.9s\\
    %RetinexFormer~\cite{cai2023retinexformer} & 24.11 & 0.78 & 5.72 & 4.60 & 1.6M & 4.2s\\
    LYT-Net~\cite{brateanu2024lyt}       & 24.19 & 0.78 & 5.64 &  1.1M & 3.9s\\
    SIRLUT~\cite{li2024sirlut}        & 24.12 & 0.78 & 5.59 & 113.3K & 2.1s\\
    %RawFormer~\cite{perevozchikov2024rawformer} & 24.21 & 0.78 & 5.49 & 4.52 & 26.1M & 6.7s\\
    cmKAN  & \colorbox{best}{25.94} & \colorbox{best}{0.89} & \colorbox{best}{4.51} & \colorbox{best}{76.4K} & \colorbox{best}{1.1s}\\
    \midrule
     & \multicolumn{3}{c|}{\colorbox{paired}{ Paired-based inference}} & \\
    %Linear (3$\times$3 matrix)    & 23.33 & 0.76 & 6.03 & 4.70 & 9 & \colorbox{best}{0.2s*}\\
    Poly~\cite{hong2001study}          & 24.27 & 0.78 & 5.08 & 57 & \colorbox{best}{0.8s*}\\ 
    Root-poly~\cite{finlayson2015color}    & 24.53 & 0.80 & 4.92 & 120 & 4.6s*\\ 
    %Homography~\cite{finlayson2017color}    & 23.29 & 0.75 & 6.05 & 5.18 & \colorbox{best}{2} & 12.8s*\\
    %Color-matcher~\cite{plenopticam} & 22.07 & 0.74 & 7.14 & 5.20 & 8 & 1.4s*\\
    NeuralPreset~\cite{ke2023neural}  & 23.35 & 0.76 & 5.97 & 5.15M & 20.4s*\\
    R.G. Rodriguez et al. ~\cite{AN2}& 24.35 & 0.78 & 4.99 & \colorbox{best}{14} & 3.3s*\\
    %SMS (Ours)    & 24.59 & 0.80 & 4.87 & 4.19 & 18 & 17.1s*\\
    %SMS, non-global (Ours)    & 25.19 & 0.?? & 4.48 & ?? & 48 & 17.1s*\\
    %KAN (Ours)    & 24.57 & 0.81 & 4.79 & 4.08 & 90 & 1.2s\\
     cmKAN-Light   & \colorbox{best}{24.57} & \colorbox{best}{0.81} & \colorbox{best}{4.79} & 7.8K & 1.5s\\
    \bottomrule
  \end{tabular}  \vspace{-2mm}
  }
\end{table}

%\begin{table}[h]
%  \centering
%  \resizebox{\linewidth}{!}
%  {
%  \begin{tabular}{@{}l|rrr@{}}
%    \toprule
%    Method        & PSNR & SSIM & $\Delta E$ \\
%    \midrule
%    Javier~\cite{AN2}       & 26.91 & 0.84 & 3.26\\
%    SMS (Ours)    & 29.15 & 0.91 & 3.14\\
%    KAN (Ours)    & 28.21 & 0.86 & 3.07\\
%    \bottomrule
%  \end{tabular}
%  }
%  \caption{Results on Javier Dataset (Reference non-free task).   Ours is better.}
%  \label{tab:cm-javier}
%\end{table}


\begin{table}[t]
  \centering
    \caption{Results of \textit{supervised} sRGB-to-sRGB mapping on the MIT-Adobe FiveK dataset~\cite{AN7}. The best-performing results are highlighted in yellow.}%Results on FiveK (480p).   Ours is better. Input for time evaluation = (3,1024,1024). * - results obtained on CPU, otherwise on GPU.}
        \vspace{-2mm}
  \resizebox{0.55\linewidth}{!}
  {
  \begin{tabular}{@{}l|ccc@{}}
    \toprule
    Method & PSNR & SSIM & $\Delta E$\\
    \midrule
    %PCE~\cite{chai2020supervised}          & 23.93 & 0.92 & 10.21 & 6.82\\
    %NeurOp~\cite{wang2022neural}        & 25.09 & 0.91 & 9.93 & 6.44\\
    %AdaInt~\cite{yang2022adaint}        & 25.49 & 0.92 & 7.47 & 5.29\\
    SepLUT~\cite{yang2022seplut}        & 25.47 & 0.92 & 7.54\\
    %RetinexFormer~\cite{cai2023retinexformer} & 24.98 & 0.92 & 7.11 & 5.22\\
    LYT-Net~\cite{brateanu2024lyt}       & 24.10 & 0.92 & 7.03\\
    SIRLUT~\cite{li2024sirlut} & 27.25 & 0.94 & 6.19\\
    cmKAN  & \colorbox{best}{31.74} & \colorbox{best}{0.95} & \colorbox{best}{2.83}\\ 
    \bottomrule
  \end{tabular}  \vspace{-4mm}
  }
  \label{tab:cm-5k}
\end{table}

%\begin{table}[t]
%  \centering
%  \caption{Results of \textit{supervised} sRGB-to-sRGB mapping on the PPR10K dataset~\cite{AN8}. We report training results using experts A, B, and C as ground-truth targets.}
%      \vspace{-2mm}
%  \resizebox{0.8\linewidth}{!}
%  {
%  \begin{tabular}{@{}l|c|c|c@{}}
%    \toprule
%    Method & PSNR / $\Delta E$ & PSNR / $\Delta E$ & PSNR / $\Delta E$\\
%    \midrule
%    & \multicolumn{1}{c|}{\colorbox{unsipervised}{Expert A}} & \multicolumn{1}{c|}{\colorbox{supervised}{Expert B}} & \multicolumn{1}{c}{\colorbox{paired}{Expert C}}\\
%    %NeurOp~\cite{wang2022neural}       & 26.46 / 8.80 & 25.82 / 8.97 & 26.23 / 8.86\\
%    %AdaInt~\cite{yang2022adaint}        & 26.33 / 6.56 & 25.40 / 7.33 & 25.68 / 7.31\\
%    SepLUT~\cite{yang2022seplut}        & 26.28 / 6.59 & 25.23 / 7.49 & 25.59 / 7.51\\
%    %RetinexFormer~\cite{cai2023retinexformer} & 00.98 / 7.11 & 23.93 / 9.21 & 23.93 / 9.21\\
%    LYT-Net~\cite{brateanu2024lyt}       & 26.10 / 7.03 & 23.93 / 9.21 & 23.93 / 9.21\\
%    SIRLUT~\cite{li2024sirlut}       & 28.31 / 5.65 & 27.67 / 5.89 & 27.79 / 6.13\\
%    cmKAN  & \colorbox{best}{32.49} / \colorbox{best}{2.21} & \colorbox{best}{32.01} / \colorbox{best}{2.35} & \colorbox{best}{32.27} / \colorbox{best}{2.77}\\ 
%    \bottomrule
%  \end{tabular}
%  }
%  %\caption{Results on PPR10K.   Ours is better. Input for time evaluation = (3,1024,1024). * - results obtained on CPU, otherwise on GPU.}
%  \label{tab:cm-ppr10k}
%\end{table}


% \subsection{Other Experiments}

% \subsubsection{raw-to-sRGB Experiments}
% TODO - write the text



% % \subsubsection{Experiments with Unpaired Data}
% % TODO - write the text


\subsection{Ablation Studies}
\vspace{-2mm}
The ablation studies in Table \ref{tab:a-studies} validate our design choices by systematically assessing key components—the KAN and Generator network. In the baseline ($C_0$), the generator uses Rawformer's encoder \cite{perevozchikov2024rawformer} with global average pooling, while the KAN is replaced with an MLP. Replacing the MLP with KAN in $C_1$ achieves a 2.29 dB improvement, highlighting KAN's importance. In $C_2$, removing average pooling for 2D generator output boosts performance further. Incremental additions to the generator—Illumination Estimator ($C_3$), Color Transformer with MSA ($C_4$), and Color Feature Modulator ($C_5$)—yield gains of 2.9 dB, 2.98 dB, and 3.33 dB, respectively, demonstrating the cumulative impact of each component.

%The results of the ablation studies, as detailed in Table  \ref{tab:a-studies}, provide a comprehensive validation of our design choices. These experiments systematically examine various configurations to assess the contributions of our key components — the KAN and the Generator network towards the overall performance enhancement.
%In the baseline configuration ($C_0$), the generator is implemented using rawformer's  encoder \cite {perevozchikov2024rawformer} with a global average pooling at the end to generate the 1D feature maps, and the KAN network being replaced by a simple multi-layer perceptron (MLP) layer. The $C_1$ configuration builds upon the baseline by substituting the MLP layers with KAN networks, resulting in an initial performance gain of 2.29 dB, thereby demonstrating the importance of incorporating KAN. The $C_2$ configuration further enhances performance by replacing the 1D generator output with a 2D output, achieved by removing the average pooling at the generator's output. %This modification enables more comprehensive feature extraction, leading to improved overall performance. 
%To achieve further refinement of the KAN output, additional components in the generator are integrated incrementally. Specifically, the Illumination Estimator ($C_3$),  Color Transformer  where we replace Rawformer's CQA with the proposed MSA ($C_4$), and Color Feature Modulator ($C_5$) are introduced sequentially. Each of these components delivers a significant performance improvement, contributing additional gains of 2.9 dB, 2.98 dB, and 3.33 dB, respectively, over the baseline. These results collectively highlight the effectiveness of our design and demonstrate the cumulative impact of each component in driving substantial improvements in the final outcomes.



%We present the ablation studies' results to validate our design choices in Table \ref{tab:a-studies}. Specifically, we evaluate different configurations to show the impact of incorporating KAN, 2D maps, the Color Transform (CT), and the Color Feature Modulator (CFM) on the final results. In this context, the baseline in \ref{tab:a-studies} refers to .... As demonstrated by the results, our proposed design achieves the best results.


\begin{table}[t]
  \centering
  \caption{Ablation study on the impact of different components of our method. Results are reported on our dataset.}
      \vspace{-2mm}
  \resizebox{0.9\linewidth}{!}
  {
  \begin{tabular}{@{}lcccccc|ccc@{}}
    \toprule
    Config & Baseline & KAN & 2D Map & IE & CT & CFM & PSNR & SSIM & $\Delta E$ \\
    \midrule
    $C_0$ & \checkmark &            &            &            &            &            & 22.61 & 0.74 & 6.41 \\
    $C_1$ & \checkmark & \checkmark &            &            &            &            & 24.90 & 0.84 & 5.10 \\
    $C_2$ & \checkmark & \checkmark & \checkmark &            &            &            & 25.23 & 0.86 & 4.71 \\
    $C_3$ & \checkmark & \checkmark & \checkmark & \checkmark &            &            & 25.51 & 0.87 & 4.65 \\
    $C_4$ & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &            & 25.59 & 0.87 & 4.58 \\
    $C_5$ & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  \colorbox{best}{25.94} &  \colorbox{best}{0.89} & \colorbox{best}{4.51} \\
    \bottomrule
  \end{tabular}
  }  \vspace{-2mm}
  \label{tab:a-studies}
\end{table}


